Dex-NeRF: Using a Neural Radiance Field to Grasp Transparent Objects

The ability to grasp and manipulate transparent objects is a major challenge for robots. Existing depth cameras have difficulty detecting, localizing, and inferring the geometry of such objects. We propose using neural radiance fields (NeRF) to detect, localize, and infer the geometry of transparent objects with sufficient accuracy to find and grasp them securely. We leverage NeRF's view-independent learned density, place lights to increase specular reflections, and perform a transparency-aware depth-rendering that we feed into the Dex-Net grasp planner. We show how additional lights create specular reflections that improve the quality of the depth map, and test a setup for a robot workcell equipped with an array of cameras to perform transparent object manipulation. We also create synthetic and real datasets of transparent objects in real-world settings, including singulated objects, cluttered tables, and the top rack of a dishwasher. In each setting we show that NeRF and Dex-Net are able to reliably compute robust grasps on transparent objects, achieving 90% and 100% grasp success rates in physical experiments on an ABB YuMi, on objects where baseline methods fail.

==> figures/dishwasher.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{@{}c@{\hspace{6pt}}c@{}}%
    \includegraphics[height=128pt]{images/dishwasher/IMG_1781_lowres.JPG} & %
    \includegraphics[height=128pt]{images/dishwasher/dishwasher_grasps.png} \\
    Camera View & Rendered Depth
    \end{tabular}
    \caption{{\bf Unloading a dishwasher}.  On the left is a cropped portion of an image of a real-world dishwasher top-rack loaded with glassware used to train the NeRF model.  The right is a depth image rendered from NeRF model and according to the intrinsics expected by Dex-Net. Three candidate grasps computed by Dex-Net are colored by their expected grasp quality (green indicates a higher quality). Several objects are difficult to see in the camera view, but show up clearly in the depth view.}
    \label{fig:dishwasher}
\end{figure*}g

==> figures/figurine_mesh.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/figurine_mesh.pdf}
    \caption{\textbf{Occupancy Detection.} Explain how the mesh is extracted. The top row is rendered using the RGB outputs and the bottom row is computed using the $\sigma$ output.}
    \label{fig:figurine_mesh}
\end{figure*}

==> figures/pipeline.tex <==
\begin{figure*}[t]
    \centering % trim = left bottom right top
    \begin{tabular}{@{}c@{\hspace{4pt}}c@{}}
         \includegraphics[height=90pt,trim=240 0 260 0,clip]{images/fetchsim/fetch_grasp_001_deer_angled_dof.png} &
         \includegraphics[height=90pt]{images/fetchsim/fetch_grasp_001_deer_angled_zoom_dof.png} \\
         \includegraphics[height=90pt,trim=240 0 260 0,clip]{images/fetchsim/fetch_grasp_002_wineglass_dof.png} & 
         \includegraphics[height=90pt]{images/fetchsim/fetch_grasp_002_wineglass_zoom_2_dof.png} \\
         \includegraphics[height=90pt,trim=240 0 260 0,clip]{images/fetchsim/fetch_grasp_002_wineglass_02_dof.png} & 
         \includegraphics[height=90pt]{images/fetchsim/fetch_grasp_002_wineglass_02_zoom_dof.png} \\
    \end{tabular}
    \includegraphics[width=\linewidth,trim=0 0 0 140,clip]{images/pipeline.pdf}
    \caption{\textbf{Using NeRF to grasp transparent objects}
    Given a scene with transparent objects (top left), we (bottom row) train a NeRF model, compute a transparency-aware depth rendering, compute a grasp with Dex-Net, and then execute the grasp.  The quality of the depth map is high enough that the grasp can be executed without unwanted collisions (top right).
    }
    \label{fig:pipeline}
\end{figure*}

==> figures/singulated_grasps.tex <==
\begin{figure*}[t]
    \centering
    % \textwidth=5.5in * 72.27pt/in = 397.485 pt
    % 397.485 - 4pt*4 = 381.485 / 5 = 76.2pt
    \begin{tabular}{@{}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{}}% trim = left bottom right top
    %\toprule
    Side view&Top-down view&Grasp 1&Grasp 2&Grasp 3 \\
    %\midrule
    {\includegraphics[width=76pt,trim=300 200 300 400,clip]{images/grasps/pipe_side_72dpi.png}}& %
    {\includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/pipe_top_72dpi.png}}& %
    {\includegraphics[width=76pt,trim=394 404 414 456,clip]{images/grasps/pipe_grasp_1_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 404 414 456,clip]{images/grasps/pipe_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 404 414 456,clip]{images/grasps/pipe_grasp_4_72dpi_c.png}} \\
    {\includegraphics[width=76pt,trim=300 200 300 400,clip]{images/grasps/pawn_side.png}}& %
    {\includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/pawn_top.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/pawn_grasp_1_72dpi.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/pawn_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/pawn_grasp_3_72dpi_c.png}} \\
    {\includegraphics[width=76pt,trim=300 200 300 400,clip]{images/grasps/turbine_housing_side.png}}& %
    {\includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/turbine_housing_top.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/turbine_housing_grasp_3_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/turbine_housing_grasp_2_72dpi.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/turbine_housing_grasp_3_72dpi_c.png}} \\
    {\includegraphics[width=76pt,trim=300 200 300 400,clip]{images/grasps/mount1_side.png}}& %
    {\includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/mount1_top.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/mount1_grasp_1_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/mount1_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/mount1_grasp_3_72dpi_c.png}} \\
    % the trim on wineglass2 is different zoom out a bit
    {\includegraphics[width=76pt,trim=300 200 300 400,clip]{images/grasps/wineglass2_side.png}}& %
    {\includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/wineglass2_top.png}}& %
    {\includegraphics[width=76pt,trim=294 300 314 352,clip]{images/grasps/wineglass2_grasp_1_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=294 300 314 352,clip]{images/grasps/wineglass2_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=76pt,trim=294 300 314 352,clip]{images/grasps/wineglass2_grasp_3_72dpi.png}} \\
    %
    \includegraphics[width=76pt,trim=300 280 300 320,clip]{images/grasps/wineglass_side.png} & %
    \includegraphics[width=76pt,trim=300 300 300 300,clip]{images/grasps/wineglass_top.png} & %
    \includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/wineglass_grasp_1_72dpi_c.png} & %
    \includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/wineglass_grasp_2_72dpi_c.png} & %
    \includegraphics[width=76pt,trim=394 400 414 452,clip]{images/grasps/wineglass_grasp_3_72dpi_c.png} \\
    %\midrule
    %Side view&Top-down view&Grasp 1&Grasp 2&Grasp 3 \\
    %\bottomrule
    \end{tabular}
    \caption{\footnotesize {\bf Grasps on singulated objects. \yahav{to save space let's keep only 1 grasp for each, and transpose this matrix. Also let's replace the image of the wineglass with the one I added to fig 3.}}  In each row, we show 2 views of a singulated object and 3 candidate grasps computed with Dex-Net. The grasps were evaluated in simulation using a wrench resistance metric that measures the ability of the grasp to resist gravity~\cite{mahler2018dex}. The grasps, colored in green for success and red for failure cases, are overlayed on the depth map generated by the proposed system. The arrows on the grasp show the closing direction of the parallel-jaw gripper fingers. The slight misalignment between the top-down view and the grasp views is due to the top-down view coming from the camera, while the depth view is generated from the NeRF model by the proposed pipeline.}
    \label{fig:singulated_grasps}
\end{figure*}

==> figures/singulated_grasps_new.tex <==
\begin{figure*}[t]
    \centering
    % \textwidth=5.5in * 72.27pt/in = 397.485 pt
    % 397.485 - 4pt*4 = 381.485 / 5 = 76.2pt
    % 397.485 - 4pt*4 = 381.485 / 6 = 63.5pt
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{}}% trim = left bottom right top
    %\toprule
    Pipe Connector&Pawn&Turbine Housing&Mount&Wineglass side&Wineglass\\
    %\midrule
    {\includegraphics[width=63pt,trim=300 200 300 400,clip]{images/grasps/pipe_side_72dpi.png}}& %
    {\includegraphics[width=63pt,trim=300 200 300 400,clip]{images/grasps/pawn_side.png}}& %
    {\includegraphics[width=63pt,trim=300 200 300 400,clip]{images/grasps/turbine_housing_side.png}}& %
    {\includegraphics[width=63pt,trim=300 200 300 400,clip]{images/grasps/mount1_side.png}}& %
    {\includegraphics[width=63pt,trim=300 200 300 400,clip]{images/grasps/wineglass2_side.png}}& %
    \includegraphics[width=63pt,trim=300 280 300 320,clip]{images/grasps/wineglass_side.png} \\
    {\includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/pipe_top_72dpi.png}}& %
    {\includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/pawn_top.png}}& %
    {\includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/turbine_housing_top.png}}& %
    {\includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/mount1_top.png}}& %
    {\includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/wineglass2_top.png}}& %
    \includegraphics[width=63pt,trim=300 300 300 300,clip]{images/grasps/wineglass_top.png} \\
    {\includegraphics[width=63pt,trim=394 404 414 456,clip]{images/grasps/pipe_grasp_4_72dpi_c.png}}& %
    {\includegraphics[width=63pt,trim=394 400 414 452,clip]{images/grasps/pawn_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=63pt,trim=394 400 414 452,clip]{images/grasps/turbine_housing_grasp_3_72dpi_c.png}}& %
    {\includegraphics[width=63pt,trim=394 400 414 452,clip]{images/grasps/mount1_grasp_2_72dpi_c.png}}& %
    {\includegraphics[width=63pt,trim=294 300 314 352,clip]{images/grasps/wineglass2_grasp_1_72dpi_c.png}}& %
    \includegraphics[width=63pt,trim=394 400 414 452,clip]{images/grasps/wineglass_grasp_1_72dpi_c.png}
    %\bottomrule
    \end{tabular}
    \caption{\footnotesize {\bf Grasps on singulated objects.}  In each row, we show 2 views of a singulated object and 3 candidate grasps computed with Dex-Net. The grasps were evaluated in simulation using a wrench resistance metric that measures the ability of the grasp to resist gravity~\cite{mahler2018dex}. The grasps, colored in green for success and red for failure cases, are overlayed on the depth map generated by the proposed system. The arrows on the grasp show the closing direction of the parallel-jaw gripper fingers. The slight misalignment between the top-down view and the grasp views is due to the top-down view coming from the camera, while the depth view is generated from the NeRF model by the proposed pipeline.}
    \label{fig:singulated_grasps}
\end{figure*}

==> figures/synthetic_grasps.tex <==
\begin{figure}[t]
    \centering
    %\includegraphics{}
    \NEW{\LARGE{TODO: New Figure.  Include: synthetic singulated object grasping (currently in supplemental material) and graph of plot}}
    \caption{\NEW{Synthetic grasping benchmarks}}
    \label{fig:synthetic_grasps}
\end{figure}
